Leaking Information Through Cache LRU States

The Least-Recently Used cache replacement policy and its variants are widely deployed in modern processors. This paper shows for the first time in detail that the LRU states of caches can be used to leak information: any access to a cache by a sender will modify the LRU state, and the receiver is able to observe this through a timing measurement. This paper presents LRU timing-based channels both when the sender and the receiver have shared memory, e.g., shared library data pages, and when they are separate processes without shared memory. In addition, the new LRU timing-based channels are demonstrated on both Intel and AMD processors in scenarios where the sender and the receiver are sharing the cache in both hyper-threaded setting and time-sliced setting. The transmission rate of the LRU channels can be up to 600Kbps per cache set in the hyper-threaded setting. Different from the majority of existing cache channels which require the sender to trigger cache misses, the new LRU channels work with the sender only having cache hits, making the channel faster and more stealthy. This paper also demonstrates that the new LRU channels can be used in transient execution attacks, e.g., Spectre. Further, this paper shows that the LRU channels pose threats to existing secure cache designs, and this work demonstrates the LRU channels affect the secure PL cache. The paper finishes by discussing and evaluating possible defenses.

==> related_work.tex <==
\section{Related Work}
\label{sec:related work}


%\subsection{Existing Cache Side and Covert Channel Attacks}


Most cache timing channels leverage the tag array.
%, such as Flush+Reload attack~\cite{yarom2014flush} and Prime+Probe attack~\cite{osvik2006cache}.
%The Flush+Reload and Prime+Probe cache channels represent two types of side and covert channels. 
The Flush+Reload attack~\cite{yarom2014flush}
transfers information by {\em reusing} the same data in the cache. There are other reuse-based cache side-channel attacks, such as
Cache Collision attack~\cite{bonneau2006cache}. The Prime+Probe attack~\cite{osvik2006cache}, on the other hand,
transfers information by creating {\em contention} in the cache.  Another example of the contention-based side channel is Evict+Time
attack~\cite{osvik2006cache}.

%Depending on whether the receiver is observing the time of his own memory accesses or the sender's memory accesses, the
%attacks are further divided into external and internal attacks~\cite{liu2014random}.
%In external attacks, the cache sharing (contention or reuse) happens between sender's execution and receiver's execution, e.g.,
%Flush+Reload and Prime+Probe.
%In internal attacks, the receiver measures the sender's execution time, and the cache contention or reuse happens within the sender's
%program, e.g., Cache Collision and Evict+Time.

Shared cache components other than the tag array have also be leveraged for side and covert channels.
For example, the contention in the cache directory in non-inclusive caches has been demonstrated and used for a side-channel
attack~\cite{yan2019attack}.
Cache coherence states have also been used to create covert channels~\cite{yao2018coherence,trippel2018meltdownprime}.

In parallel to this work, there is a recent {\em arXiv} preprint paper~\cite{briongos2019reload} on side channels that leverage the replacement policy in LLC,
where shared memory is required. However, we demonstrate the LRU channels both with and without shared memory. 
Their attack also relies on {\em clflush} instruction and their use of flush operation cannot be replaced by a series of memory accesses (as we do in our attack),
which makes the attack unpractical in settings where {\em clflush} is not available, e.g., in JavaScript.
Further, L1 is directly accessed by the processor pipeline and local cache accesses will not cause updates in the LLC replacement states used in~\cite{briongos2019reload}, so our attack is more stealthy and any LLC defenses do not stop our attack.


%\subsection{Cache Side Channel Mitigations}
%
Due to the threat of the various timing channels, many secure cache designs have been proposed in the literature to defend the attacks~\cite{lee2005architecture,wang2007new,domnitser2012non,zhang2012language,yan2017secure,kiriansky2018dawg,costan2016sanctum},
as already discussed in Section~\ref{sec_lru_and_sec_caches}.
%Again, partitioning based designs~\cite{lee2005architecture,wang2007new,domnitser2012non,zhang2012language,yan2017secure,kiriansky2018dawg,costan2016sanctum,liu2014random,liu2016newcache,keramidas2008non}
%and randomization based design~\cite{liu2014random,liu2016newcache,keramidas2008non} exists.
However, most do not have, or did not consider, LRU attacks and cannot defend against them.
%
%Other secure cache designs~\cite{liu2014random,liu2016newcache,keramidas2008non} use randomization to decouple the cache
%states and memory access history by the sender. In this way, the receiver's observation of cache state is not related to the sender's
%memory access pattern.
%Meanwhile

Another approach is to use hardware performance counters to detect a potential cache side channel attacks in
real time,~\cite{zhang2016cloudradar,chiappetta2016real,alam2017performance}, because the root cause of the existing cache side channel is cache misses.
However, the LRU channels require either hits or misses, so counting misses of the sender only will not detect the attack.


%\textbf{FIXME somewhere need to mention the related work that partitions LRU states, Sanctum?}




